The First Principles of Deep Learning and Compression

The deep learning revolution incited by the 2012 Alexnet paper has been transformative for the field of computer vision. Many problems which were severely limited using classical solutions are now seeing unprecedented success. The rapid proliferation of deep learning methods has led to a sharp increase in their use in consumer and embedded applications. One consequence of consumer and embedded applications is lossy multimedia compression which is required to engineer the efficient storage and transmission of data in these real-world scenarios. As such, there has been increased interest in a deep learning solution for multimedia compression which would allow for higher compression ratios and increased visual quality. The deep learning approach to multimedia compression, so called Learned Multimedia Compression, involves computing a compressed representation of an image or video using a deep network for the encoder and the decoder. While these techniques have enjoyed impressive academic success, their industry adoption has been essentially non-existent. Classical compression techniques like JPEG and MPEG are too entrenched in modern computing to be easily replaced. This dissertation takes an orthogonal approach and leverages deep learning to improve the compression fidelity of these classical algorithms. This allows the incredible advances in deep learning to be used for multimedia compression without threatening the ubiquity of the classical methods. The key insight of this work is that methods which are motivated by first principles, i.e., the underlying engineering decisions that were made when the compression algorithms were developed, are more effective than general methods. By encoding prior knowledge into the design of the algorithm, the flexibility, performance, and/or accuracy are improved at the cost of generality...

==> appendices/study/tables/forensics_full.tex <==
\begin{tabular}{llllrrrrrrrrr}
    \toprule
    Model                        & Metric                          & Reference              & Mitigation                        & Q=10  & Q=20  & Q=30  & Q=40  & Q=50  & Q=60  & Q=70  & Q=80  & Q=90  \\
    \midrule
    \multirow{4}{*}{Chai et. al} & \multirow{4}{*}{Patch Accuracy} & \multirow{4}{*}{93.83} & Supervised Fine-Tuning            & 53.04 & 54.81 & 56.12 & 56.86 & 57.34 & 57.66 & 58.07 & 58.58 & 59.41 \\
                                 &                                 &                        & None                              & 49.87 & 49.46 & 49.48 & 49.86 & 50.33 & 50.74 & 51.12 & 51.83 & 53.26 \\
                                 &                                 &                        & Off-the-Shelf Artifact Correction & 50.56 & 50.20 & 50.34 & 50.63 & 51.14 & 51.63 & 52.26 & 53.22 & 54.12 \\
                                 &                                 &                        & Task-Targeted Artifact Correction & 51.99 & 52.46 & 52.70 & 52.98 & 53.21 & 53.33 & 53.48 & 53.58 & 53.28 \\
    \midrule
    \multirow{4}{*}{Wang et. al} & \multirow{4}{*}{Accuracy}       & \multirow{4}{*}{99.96} & Supervised Fine-Tuning            & 89.70 & 96.69 & 98.41 & 99.04 & 99.44 & 99.54 & 99.65 & 99.88 & 99.91 \\
                                 &                                 &                        & None                              & 54.25 & 91.08 & 97.56 & 98.79 & 99.28 & 99.38 & 99.60 & 99.81 & 99.84 \\
                                 &                                 &                        & Off-the-Shelf Artifact Correction & 50.00 & 50.00 & 50.00 & 50.00 & 50.00 & 50.00 & 50.00 & 50.00 & 50.00 \\
                                 &                                 &                        & Task-Targeted Artifact Correction & 50.00 & 50.00 & 50.00 & 50.00 & 50.00 & 50.00 & 50.00 & 50.00 & 50.00 \\
    \bottomrule
\end{tabular}

==> chapters/image_compression/qgac/empirical.tex <==
\section{Empirical Evaluation}
No artifact correction work is complete without an empirical evaluation, and with the algorithm now developed, we are in a position to perform one. For this evaluation we train the network using the Adam \sidecite{kingma2014adam} optimizer using a batch of 32 $256 \times 256$ patches, the network is implemented in PyTorch \sidecite{NEURIPS2019_9015}. All DCT coefficients are normalized using per-channel and per-frequency mean and standard deviations. quantization matrices are normalized to $[0, 1]$ and use the ``baseline'' setting in libjpeg \sidecite{libjpeg}.

The training proceeds in stages, as described previously. First the Y channel network is trained using $\Lagr_R$ (\refeq{loss_r}) for 400,000 batches with the learning rate starting at $10^{-3}$ and decaying by a factor of 2 every 100,000 batches. We set $\lambda = 0.05$. Then we freeze the Y channel weights and train the color network using $\Lagr_R$ (\refeq{loss_r}) for 100,000 batches with the learning rate decaying from $10^{-3}$ to $10^{-6}$ using cosine annealing \sidecite{loshchilov2016sgdr}.

With the network fully trained for regression we then fine-tune end-to-end using $\Lagr_\text{GAN}$ (\refeq{loss_g}). The network is again trained for 100,000 iterations using cosine annealing this time with the learning rate starting at $10^{-4}$ and ending at $10^{-6}$. We set $\gamma = 5 \times 10^{-3}$ and $\nu = 10^{-2}$.

For training data we use DIV2k and Flickr2k \sidecite{agustsson2017ntire} which contain 900 and 2650 images respectively. We pre-extract 30 $256 \times 256$ patches from each image and compress them using quality in $[10, 100]$ in steps of 10 for a total training set size of 1,065,000 patches. We evaluate the method using the Live1 \sidecite{sheikh2006statistical}, Classic-5 \sidecite{foi2006pointwise}, and ICB \sidecite{icb} datasets. To be consistent with prior works, we report PSNR, PSNR-B, and SSIM as metrics for the regression network. For the GAN we report FID score \sidecite{heusel2017gans}.

\subsection{Comparison with Other Methods}
\labsec{qgac-comparisons}

We start by comparing our method to others in the form of a large boring table in \reftab{qgac-quant}. Note that this uses the regression weights only. Note that of the compared methods, only IDCN has native handling of color information and all of the methods are quality dependent with a different model for each quality. Ours, in contrast, is only a single model.

\begin{table*}[t]
    \centering
    \caption[QGAC Quantitative Results]{\textbf{QGAC Quantitative Results.} Format is PSNR (dB)$\uparrow$ / PSNR-B (dB) $\uparrow$ / SSIM $\uparrow$ with the best result shown in bold. This table is provided for those dedicated enough to read the small font. These numerical results are unimportant; what is important is the qualitative results that follow.}
    \resizebox{1.5\textwidth}{!}{
        \input{tables/color_results.tex}
    }
    \labtab{qgac-quant}
\end{table*}

\subsection{Generalization}
\labsec{qgac-generalize}

In the development of this method we place emphasis on a single network generalizing to multiple JPEG qualities. This raises an interesting question: ``can other models generalize to different qualities?'' In general the answer is ``no'' and we demonstrate this using IDCN \sidecite{zheng2019implicit} with an example image compressed at quality 50. Since IDCT provides only quality 10 and 20 models, we test both of those models on this image. The result is shown in \reffig{qgac-generalize}. The quality 10 model oversmoothes this image and it appears worse than the JPEG it was supposed to correct. The quality 20 model looks better, but QGAC's single model looks the best as it was able to adapt its weights to the quality 50 JPEG by processing the quantization data. As this experiment shows, it is important for prior works to select the correct model for the JPEG.
\begin{figure*}[t]
    \centering
    \includegraphics{figures/generalize.pdf}
    \caption[Quality Generalization]{\textbf{Quality Generalization.} Note that both the IDCN quality 10 and 20 models appear to oversmooth the quality 50 JPEG.}
    \labfig{qgac-generalize}
\end{figure*}

\begin{marginfigure}[-5\baselineskip]
    \centering
    \includegraphics{figures/increase.pdf}
    \caption[Increase in PSNR]{\textbf{Increase in PSNR.} Shown for color datasets on all JPEG quality settings. Note the steep dropoff at high qualities.}
    \labfig{qgac-increase}
\end{marginfigure}

In fact, since our method is not restricted in quality, we can show how it generalizes in an even more compelling way: by testing on all JPEG quality settings. We show this in the graph in \reffig{qgac-increase}. Note that for most quality settings, the increase is fairly stable, only at quality 90 and above does a steep dropoff occur. For these qualities, however, the degradation is hardly noticeable and artifact correction is likely not necessary.

\subsection{Equivalent Quality}

One important application of artifact correction is to improve compression fidelity. In other words, rather than replacing the entire JPEG codec with a compression algorithm based on deep learning, we can simply use more aggressive JPEG settings and use artifact correction to make the result presentable. This is much more likely to succeed in the short term due to the technical debt surrounding JPEG.

\begin{marginfigure}
    \centering
    \includegraphics{figures/eq_qual_plots.pdf}
    \caption[Equivalent Quality Plots]{\textbf{Equivalent Quality Plots.} Top: space savings on average. Bottom: equivalent quality on average.}
    \labfig{qgac-eq}
\end{marginfigure}

We explore this phenomenon using ``equivalent quality'', \ie, given a JPEG which is compressed at some low quality and then corrected, what higher quality would we have had to compress the image at in order to match the restored error? And how much space did we save by using the smaller JPEG image? We start with an example in \reffig{qgac-eq-ex}.

Note that our model is equivalent to almost doubling the quality of the JPEG, allowing us to save a significant amount of space. Next we compute the equivalent quality over the entire Live1 dataset and plot it along with the space savings in kB. We do this for qualities 10-50. These plots are shown in \reffig{qgac-eq}.

\begin{figure*}[t]
    \centering
    \includegraphics{figures/eq_qual.pdf}
    \caption[Equivalent Quality Examples]{\textbf{Equivalent Quality Examples.} Taking three images compressed at random qualities, we correct them and then find the compression quality that matches the corrected result in terms of error.}
    \labfig{qgac-eq-ex}
\end{figure*}

\subsection{Exploring Convolutional Filter Manifolds}
\labsec{qgac-cfm-res}

\begin{figure}[t]
    \centering
    \includegraphics{figures/tsne.pdf}
    \caption[Embeddings for Different CFM Layers.]{\textbf{Embeddings for Different CFM Layers.} 3 channels are taken from each embedding, color shows JPEG quality
        setting that produced the input quantization matrix. Circled
        points indicate quantization matrices that were seen during training.}
    \labfig{quality_tsne}
\end{figure}

Of the various proposals in this work, one of the most intriguing is the Convolutional Filter Manifold (CFM). In this section we explore their properties empirically. First we can visualize the CFM weights. We do this by pulling out three channels of one of the CFM layers. Since we can adapt these weights, we generate quantization matrices for qualities 10, 50, and 100 and produce CFM weights. This is shown with a heatmap in \reffig{qgac-cfm-weight-vis}.

\begin{figure}[p]
    \centering
    \includegraphics{figures/cfm_weights.pdf}
    \caption[CFM Weight Visualization.]{\textbf{CFM Weight Visualization.} Horizontal axis shows different channels of the weight, vertical
        axis shows quality. Quality levels shown are Top: 10, Middle: 50, Bottom: 100. These are simply the heatmapped $8 \times 8$ kernels of the CFM layer.}
    \labfig{qgac-cfm-weight-vis}
\end{figure}

We see some interesting behavior in this figure. The kernels in each row appear different, since these are different channels we hope that they are different as they should capture different information. In contrast, the kernels in each column appear to be similar, but scaled versions with the magnitude decreasing as quality increases. This makes sense because high quality images should need less correction.

We can take this visualization further by finding the filters which maximally activate each of these weights. This will tell us which patterns each filter responds to. We do this by taking a noise image and optimizing it to maximize the output of the filter. In other words, we treat the visualization as a parameter and use stochastic gradient ascent with the objective being the magnitude of the weight we wish to visualize. This result is shown in \reffig{qgac-cfm-max-activation}.

We again see some interesting behavior. Clear patterns of JPEG artifacts are visible in these images. As in \reffig{qgac-cfm-weight-vis}, the columns seem to capture different types of artifacts, with the first column capturing local block artifacts, the second capturing larger block artifacts, and the the third capturing some ringing artifacts. As we descend each column, we see similar artifacts reducing in strength until the quality 100 filter which leaves the images mostly unchanged.

\begin{figure}[p]
    \centering
    \includegraphics{figures/cfm_act.pdf}
    \caption[Images Which Maximally Activate CFM Weights.]{\textbf{Images Which Maximally Activate CFM Weights.} Horizontal axis shows
        different channels from the weight, vertical axis shows quality. Quality levels shown are Top: 10, Middle: 50, Bottom: 100.}
    \labfig{qgac-cfm-max-activation}
\end{figure}

Finally, we can examine the manifold property of the CFM. We show this in \reffig{quality_tsne} where we have taken the three kernels from three different CFM layers for all possible quantization matrices (0-100). We then compute a t-SNE embedding \sidecite{hinton2002stochastic} to two dimensions and plot the kernels. What we see is a smooth manifold through the space of quantization matrices. By coloring each point by the quality level used to generate it, we can see that the kernels generate an order on the space. We can also see that each channel corresponds to a different manifold.

\subsection{Frequency Domain Results}

Next we analyze the constituent frequencies of compressed and restored images. One of the claims we made when developing the method is that GAN training produced more realistic high frequency reconstructions. Indeed, by examining \reffig{qgac:freq} we can see that, compared with JPEG and regression reconstruction, the GAN result has significantly more activity in the high frequencies. We show this both with heatmaps of the Y channel coefficients and by plotting the ``probability'' \sidenote{We use the definition of frequency $m$ such that $i + j = m$ for a 2D frequency $(i,j)$ for simplicity.}  with which a given frequency is non-zero on a bar chart, for four examples. Examining the frequency chart, we can see that in real images, even the highest frequency components have some probability of being non-zero. This probability is significantly reduced by JPEG compression and the regression result does little to correct it. The GAN result on the other hand has high frequency responses that are significantly higher, at least as likely to be non-zero as the original images. So in this sense at least, the GAN loss was successful.

\begin{figure*}[p]
    \centering
    \includegraphics[width=1.5\textwidth]{figures/freq_woman.pdf}
    \caption[Frequency Domain Results]{\textbf{Frequency Domain Results.} Note how the GAN reconstruction generates significantly more high frequency content than the regression reconstruction. Also note how few high frequencies are in the compressed image. We show only one example here, please see more examples in Appendix \ref{app:ar}.}
    \labfig{qgac:freq}
\end{figure*}

\subsection{Qualitative Results}

In this section we simply show some qualitative outputs of the model, these results are shown in \reffig{qgac:qual}. Observe that the degraded images suffer from extreme banding caused by the quantization process. Our reconstructions are able to effectively mitigate this banding, along with other complex ringing and blocking artifacts. More qualitative results are given in Appendix \ref{app:ar}.

\begin{figure*}[p]
    \centering
    \includegraphics[width=1.5\textwidth]{figures/qual_small.pdf}
    \caption[Qualitative Results]{\textbf{Qualitative Results.} The compressed images at quality 10 are compared to our reconstructions and the originals.}
    \labfig{qgac:qual}
\end{figure*}

==> chapters/image_compression/qgac/tables/color_results.tex <==
\begin{tabular}{@{}r *{7}{l}@{}}
    \toprule
    Dataset                  & Quality & JPEG                  & ARCNN \parencite{dong2015compression} & MWCNN \parencite{liu2018multi} & IDCN \parencite{zheng2019implicit} & DMCNN \parencite{zhang2018dmcnn} & QGAC (Ours)                    \\
    \midrule
    \multirow{3}{*}{Live-1}  & 10      & 25.60 / 23.53 / 0.755 & 26.66 / 26.54 / 0.792                 & 27.21 / 27.02 / 0.805          & 27.62 / 27.32 / 0.816              & 27.18 / 27.03 / 0.810            & \textbf{27.65 / 27.40 / 0.819} \\
                             & 20      & 27.96 / 25.77 / 0.837 & 28.97 / 28.65 / 0.860                 & 29.54 / 29.23 / 0.873          & \textbf{30.01} / 29.49 / 0.881     & 29.45 / 29.08 / 0.874            & 29.92 / \textbf{29.51 / 0.882} \\
                             & 30      & 29.25 / 27.10 / 0.872 & 30.29 / 29.97 / 0.891                 & 30.82 / 30.45 / 0.901          & -                                  & -                                & \textbf{31.21 / 30.71 / 0.908} \\
    \midrule
    \multirow{3}{*}{BSDS500} & 10      & 25.72 / 23.44 / 0.748 & 26.83 / 26.65 / 0.783                 & 27.18 / 26.93 / 0.794          & 27.61 / 27.22 / 0.805              & 27.16 / 26.95 / 0.799            & \textbf{27.69 / 27.36 / 0.810} \\
                             & 20      & 28.01 / 25.57 / 0.833 & 29.00 / 28.53 / 0.853                 & 29.45 / 28.96 / 0.866          & \textbf{29.90} / 29.20 / 0.873     & 29.35 / 28.84 / 0.866            & 29.89 / \textbf{29.29 / 0.876} \\
                             & 30      & 29.31 / 26.85 / 0.869 & 30.31 / 29.85 / 0.887                 & 30.71 / 30.09 / 0.895          & -                                  & -                                & \textbf{31.15 / 30.37 / 0.903} \\
    \midrule
    \multirow{3}{*}{ICB}     & 10      & 29.31 / 28.07 / 0.749 & 30.06 / 30.38 / 0.744                 & 30.76 / 31.21 / 0.779          & 31.71 / 32.02 / 0.809              & 30.85 / 31.31 / 0.796            & \textbf{32.11 / 32.47 / 0.815} \\
                             & 20      & 31.84 / 30.63 / 0.804 & 32.24 / 32.53 / 0.778                 & 32.79 / 33.32 / 0.812          & 33.99 / 34.37 / 0.838              & 32.77 / 33.26 / 0.830            & \textbf{34.23 / 34.67 / 0.845} \\
                             & 30      & 33.02 / 31.87 / 0.830 & 33.31 / 33.72 / 0.807                 & 34.11 / 34.69 / 0.845          & -                                  & -                                & \textbf{35.20 / 35.67 / 0.860} \\
    \bottomrule
\end{tabular}

==> chapters/video_compression/dl/dl.tex <==
\setchapterpreamble[u]{\margintoc}
\chapter{Improving Video Compression}
\labch{dl-vid}

\lettrine{F}{ollowing} the same model as \nrefch{dl-jpeg}, we now survey techniques for improving video compression using deep learning. Compared with JPEG compression, this chapter will seem quite short. Video methods are still somewhat of a novelty in deep learning literature as of the time of writing, and the subfield of video compression reduction\index{video compression reduction} is particularly nascent. One major difference between JPEG and video compression is the inclusion of the in-loop deblocking filter\index{in-loop filter}. Although some JPEG software does use rudimentary heuristic deblocking, all modern video codecs include reasonably effective deblocking filters. However, these filters are not perfect and often there are still visible artifacts, although this filter does complicate the task for the network quite a bit.

The field can be divided into two disjoint sets. The first set of methods, single frame methods, consider only a single video frame at a time. They may act differently on different types of frames (\eg, I- or P-frames) but they never consider information from any previous or future frame. Multi-frame methods in contrast do consider several frames. While general restoration techniques have largely moved from sliding-window to recurrent methods thanks to the significant efficiency improvements of the recurrent models, video compression reduction methods still use sliding windows.

Before reviewing these methods we will first discuss four important works in general video restoration. These are methods which are so influential that they have had an outsize effect on the entire restoration field and thus should be considered critical background knowledge. We will then proceed to study only video compression reduction methods.

\begin{warningbox}
    Get ready for another, albeit shorter, history lesson
\end{warningbox}

\section{Notable Methods for General Video Restoration}

More general video restoration methods have a long history particularly in super-resolution. For our purposes we will only examine works of outsize importance such that they have highly influenced followup works in video compression reduction. These are all methods which combine information from multiple frames, a distinguishing feature of video restoration \vs image restoration.

The first work we discuss is FRVSR \sidecite{frvsr}. FRVSR is notable for its highly efficient recurrent formulation. This came at a time when video restoration was either single frame or was using sliding windows. Sliding windows should offer better performance but are significantly more resource intensive to compute. The lightweight recurrent formulation was a significant step towards the practical application of these techniques.

The next year ToFlow \sidecite{Xue_Chen_Wu_Wei_Freeman_2019} was published. A common idea in video restoration methods is that consecutive frames, or their features, must be aligned in order to make proper use of the extra information, and this is commonly done with optical flow. The key insight of ToFlow is that that optical flow can be learned using a network which is trained as part of the restoration process, customizing the optical flow to the task. Another major contribution of this paper is the Vimeo90k dataset which is widely used in video restoration literature.

In the same year came the next major innovation in video enhancement: EDVR \sidecite{Wang_Chan_Yu_Dong_Loy_2019}. The main contribution of EDVR was the replacement of explicit motion compensation with optical flow with implicit motion compensation using deformable convolutions. The deformable convolutions allow the feature extraction network to automatically capture information which is spatially offset in frames to account for motion. This should be a faster and more flexible method than optical flow; however, the ~20M parameter model and seven frame sliding window was highly impractical.

Finally we discuss the COMISR \sidecite{Li_Jin_Yang_Liu_Yang_Milanfar_2021} method. COMISR is a recurrent super-resolution method with a specific focus on compressed video. Li \etal rightly observe that real videos are compressed and yet prior restoration work does not take this into account. Their method is trained and tested on compressed videos and includes a novel Laplacian loss which is designed to restore high frequency details.

\section{Single Frame Methods}

As early as 2017, single frame methods were presented for video compression reduction. These methods are quite simple and only account for information in the frame that is currently being restored. Unlike the general restoration methods presented in the previous section there is no dependence on additional information from prior or future frames.

DCAD \sidecite{wang2017novel} proposed a simple method for restoring single frames of HEVC compressed video. The method bears a striking resemblance to ARCNN \sidecite{dong2014learning}. The method uses a stack of convolutional layers. The main point of comparison is the built in deblocking filter which they show an improvement over.

The QE-CNN \sidecite{yang2018enhancing} method presented the next year was designed to take compression into account explicitly. This is done using two networks, QE-CNN-I for I-frames and QE-CNN-P for P-frames. Interestingly, for P-frames, the method applies both the -I network and the -P network as HEVC encoding may contain intra- and inter- slices in one P-frame. Note that these networks still only consider a single frame at a time even though separate networks are used for the I- and P-frames; there is no shared hidden state or window.

\begin{table*}[t]
    \centering
    \caption[Summary of Video Compression Reduction Techniques]{\textbf{Summary of Video Compression Reduction Techniques.} Methods are listed with their use of multiple frames and their method for motion compensation in publication order.}
    \resizebox{1.5\textwidth}{!}{
        \begin{tabular}{llllll}
            \toprule
            Year & Name     & Citation                               & Multi-frame                         & Motion Compensation & Note                              \\
            \midrule
            2017 & DCAD     & \cite{wang2017novel}                   & \textcolor{BrickRed}{$\times$}      & -                   &                                   \\
            2018 & QE-CNN   & \cite{yang2018enhancing}               & \textcolor{BrickRed}{$\times$}      & -                   & Separate I- and P-frames networks \\
                 & MFQE     & \cite{Yang_Xu_Wang_Li_2018}            & \textcolor{JungleGreen}{\checkmark} & Explicit            & PQFs (SVM)                        \\
            2020 & STDF     & \cite{Deng_Wang_Pu_Zhuo_2020}          & \textcolor{JungleGreen}{\checkmark} & Implicit            &                                   \\
            2021 & MFQE 2.0 & \cite{Xing_Guan_Xu_Yang_Liu_Wang_2021} & \textcolor{JungleGreen}{\checkmark} & Explicit            & PQFs (BiLSTM)                     \\
                 & PTSQE    & \cite{ding2021patch}                   & \textcolor{JungleGreen}{\checkmark} & Implicit            & 3D Convolution                    \\
                 & RFDA     & \cite{zhao2021recursive}               & \textcolor{JungleGreen}{\checkmark} & Implicit            & Cross-window recurrent            \\
            \bottomrule
        \end{tabular}
    }
    \labtab{dl-vid:summary}
\end{table*}

\section{Multi-Frame Methods}

In 2018, MFQE \sidecite{Yang_Xu_Wang_Li_2018}, the first multi-frame video compression reduction network, was developed. In addition to the seven frame sliding window with optical flow alignment, this method introduced the concept of peak quality frames\index{peak quality frame} (PQFs). PQFs are frames which naturally have a higher quality than their surrounding frames and therefore have more information to extract. MQFE leverages these frames by extracting feature from them separately and using those features to guide the restoration of the nearby non-PQFs. They identify the PQFs by manually labeling frames by PSNR and then training an SVM. At test time, the SVM identifies PQFs, then the PQF features are extracted, and finally the entire sequence is restored in a sliding window. The followup work, MFQE V2 \sidecite{Xing_Guan_Xu_Yang_Liu_Wang_2021} replaces the SVM with a Bi-LSTM \sidecite{schuster1997bidirectional} which is more accurate. In addition to these ideas the MFQE paper also introduces the dataset which is used for all follow-up works.

STDF \sidecite{Deng_Wang_Pu_Zhuo_2020} is the next major advancement. This method takes the key idea from EDVR - deformable convolutions - and applies it to compression artifact reduction. The network consists of offset prediction, deformable feature extraction, and quality enhancement modules.

The following year, PTSQE \sidecite{ding2021patch}, a patch-based method, was introduced. The key idea is to use separate networks for capturing spatial and temporal information of a single patch and to use attention methods to fuse the two. PTSQE also takes the step of incorporating the residual dense blocks from ESRGAN \sidecite{wang2018esrgan}. The implicit motion compensation is also done using 3D convolutions instead of the traditional deformable convolution.

Finally, RFDA \sidecite{zhao2021recursive}, another recent model, uses a recursive fusion method to artificially increase the temporal window size. The method is built on the STDF method, and uses STDF wholesale as a subnetwork. From the STDF output, the method outputs a hidden state which is used in a downstream network to hold additional information from prior sliding windows. In this way, the STDF model is essentially accessing additional temporal information. This is almost a recurrent method in its function although the STDF method is still sliding window.

\section{Summary and Open Problems}

The methods discussed in this section are summarized in \reftab{dl-vid:summary}. At a high level, the summary is that multi-frame methods are preferred to single frame methods (because of their increased performance), and implicit motion compensation is preferred to explicit because it is faster to compute.

Given these high level ideas, there are some outstanding problems we can identify. First, it is interesting to note that the implicit motion compensation performs as well if not better than explicit (optical flow based) motion compensation. This implies that fine grained alignment may not be completely necessary for enhancement, or at least for video compression reduction. This finding was at least partially confirmed by ToFlow which showed that a task guided flow is better than a ``perfect'' flow.

On a related note, although QE-CNN was aware of the underlying metadata of frame type, there is otherwise a lack of use of bitstream metadata. This is surprising since the bitstream information often contains useful cues for how information was removed from the original frames. Additionally, coarse motion information is present in the metadata which, as we already discussed, may be good enough for feature alignment. In the next chapter, we will develop a video compression reduction method which addresses these issues.

==> chapters/video_compression/metabit/empirical.tex <==
\section{Empirical Evaluation}

With the method sufficiently developed we can empirically evaluate its performance. In all cases we train our network using the MFQE training split \sidecite{Yang_Xu_Wang_Li_2018} which consists of 108 variable length sequences. To this we add a randomly selected one third of the Vimeo90k dataset \sidecite{Xue_Chen_Wu_Wei_Freeman_2019} which is approximately 30,000 7-frame sequences. We randomly crop $256 \times 256$ patches (and 7 frames from the MFQE examples) and apply random vertical and horizontal flipping during training. For H.264 bechmarks we encode using one I-frame and six P-frames with CRF encoding as discussed in the previous section. For H.265 benchmarks we comply with prior works and use CQP encoding. We train a separate model for each QP or CRF setting. All evaluations are conducted on the MQFE test split of 18 variable length sequences.

The network is implemented in PyTorch \sidecite{NEURIPS2019_9015} and optimized using the Adam \sidecite{kingma2014adam} optimizer for 200 epochs with the learning rate set to $10^{-4}$. For quantitative experiments we train using the regression loss (\refeq{mb:regloss}) with $\alpha = [1.0\;1.0]$. For qualitative results we fine tune using the GAN loss (\refeq{mb:ganloss}) for an additional 200 epochs with a learning rate of $10^{-5}$ and $\beta = [0.01\; 0.01\; 0.005\; 1]$. As recommended we use the RMSProp optimizer for Wassertein GAN training \sidecite{arjovsky2017wasserstein}.

For numerical results we report the change in PSNR and the change in LPIPS \sidecite{zhang2018unreasonable}. For compared works we only compute LPIPS if there is a published model or training code. We find no usable trend in SSIM \sidecite{wang2004image} so we do not report that although some other works do. For consistency with prior work we report metrics on the Y channel only although we would like to see this practice end soon. To evaluate the GAN, besides providing qualitative results we report FID \sidecite{heusel2017gans} and LPIPS.

\subsection{Restoration Evaluation}

We start with the boring numerical results in \reftab{mb:hevc} for HEVC and \reftab{mb:avc} for AVC. We can see that the Metabit architecture we developed has a significantly better reconstruction result in most cases. The only exceptions are in the high QPs for HEVC where our method ties the next most recent work. For AVC, the results are significantly better indicating that the more complex CRF degradation is handled well by our method, in other words, the extra parameterization is able to better model complex degradations. Note that MFQE failed to converge entirely for CRF training. Note that PTSQE \sidecite{ding2021patch} does not provide public code and RFDA \sidecite{zhao2021recursive} does not provide usable training code so we were unable to fully evaluate these methods.

\begin{table}[t]
    \centering
    \caption[Metabit HEVC Results]{\textbf{Metabit HEVC Results.} Reported as $\Delta$PSNR (dB) $\uparrow$ / $\Delta$LPIPS $\downarrow$.}
    \resizebox{\textwidth}{!}{
        \input{tables/h265}
    }
    \labtab{mb:hevc}
\end{table}

\begin{table}[t]
    \centering
    \caption[Metabit AVC Results]{\textbf{Metabit AVC Results.} Reported as $\Delta$PSNR (dB) $\uparrow$ / $\Delta$LPIPS $\downarrow$.}
    \resizebox{\textwidth}{!}{
        \input{tables/h264}
    }
    \labtab{mb:avc}
\end{table}

\begin{margintable}
    \centering
    \caption[Metabit GAN Numerical Results]{\textbf{Metabit GAN Numerical Results.} Reported as FID $\downarrow$ / LPIPS $\downarrow$}
    \resizebox{\textwidth}{!}{
        \input{tables/gan.tex}
    }
    \labtab{mb:fid}
\end{margintable}

To evaluate the GAN we report FID and LPIPS in \reftab{mb:fid}. Note that this compares the degraded AVC input with our model trained for regression \vs GAN on extreme CRF settings (40, 50), we do not bother comparing to other works. As expected, the GAN generates significantly more realistic results.

\begin{marginfigure}
    \centering
    \includegraphics[width=\textwidth]{figures/fps-params.pdf}
    \caption[FPS \vs Params]{\textbf{FPS \vs Params.} The size of each point indicates the increase in PSNR.}
    \labfig{mb:fpsparams}
\end{marginfigure}
A more important numerical result for our purposes is throughput, specifically when compared with the number of model parameters. Our formulation is designed to be highly efficient while permitting a large number of parameters, traits which are important for timely and accurate video restoration. This result is shown graphically in \reffig{mb:fpsparams}. We see that our method is as fast as STDF with about double the parameters and a higher PSNR. In other words, our method is able to better utilize the extra parameters without slowing down thanks to the efficiency improvements we made by leveraging the bitstream metadata.

With the numerical results out of the way we can look at how the restoration functions on real images, with an example shown in \reffig{mb:bbb} from the short film Big Buck Bunny \sidecite{bbb}. In this example we can see that despite the heavy compression (ACV CRF 40), the multiframe GAN restoration is able to produce a striking resemblance to the original image. Textures are accurately reconstructed on the grass and tree and yet the smooth sky region is preserved, \ie, the network has not hallucinated textures where thy should not be. This is even more remarkable considering that there was no artificial training data.

To compare the effect of GAN restoration we show crops in \reffig{mb:compare}. The difference here is quite pronounced. Although STDF and Metabit using regression are able to improve the visual quality of the images, the GAN restoration is significantly more realistic in terms of overall sharpness and texture. This is particularly noticeable on the trees in the top row.


\subsection{Compression Evaluation}

As in \nrefch{qgac} one of the principal applications of restoration is as a method to better compress media. For our case, we can make a direct comparison to other fully deep learning based compression codecs where we compare quite favorably both in terms of latency and rate-distoration.

\begin{marginfigure}
    \centering
    \includegraphics{figures/rd.pdf}
    \caption[Rate-Distortion Comparison]{\textbf{Rate-Distortion Comparison.} Using Metabit with AVC compression performs better for low bitrates than fully deep learning codecs. Distortion is measured using PSNR.}
    \labfig{mb:rd}
\end{marginfigure}

\begin{marginfigure}
    \centering
    \includegraphics{figures/fps-lc.pdf}
    \caption[Learned Compression Throughput Comparison]{\textbf{Learned Compression Throughput Comparison.} Orange shows encoding time, blue shows decoding time. Current fully deep learning based codecs are quite slow. One major advantage of using video restoration is that encoding is quite fast. Decoding is on par with other methods except NeRV, although NeRV has a much slower encoding time.}
    \labfig{mb:fps-lc}
\end{marginfigure}

The rate-distortion result is shown in \reffig{mb:rd} along with with a number of recent deep learning based compression algorithms. We use the UVG dataset \sidecite{mercat2020uvg} for this task, which is a widely used dataset for compression evaluation. We compare to \cite{wu2018video}, \cite{lu2019dvc}, \cite{liu2020conditional}, \cite{chen2021nerv}, \cite{yang2020hierarchical}, \cite{yang2020learning}, and \cite{agustsson2020scale}. Note that we use a model trained for regression only in this case.

One potential problem we encounter here is that deep learning based compression literature compares with ``low-delay P''\index{low-delay p mode} mode compression. This is a compression setting which saves additional space by using only a single I-frame for the entire sequence with the rest of the frames encoded as P-frames. This setting saves additional space over placing I-frame periodically at the cost of quality and is often used in streaming scenarios where low-latency is critical. In order to compare fairly, we modify our restoration procedure slightly to accommodate this. Since the first group of seven frames always includes an I-frame, this group is restored following our standard procedure. We then cache the restored seventh P-frame and instead of reading seven more frames we read six. These six frames are all P-frames and we use the cached restored P-frame in place of an I-frame. There is no retraining of the network involved in this process so the results are likely lower than they could be if we trained for this scenario; however this likely improves cross-block temporal consistency by reusing information from the previous block.

For low bitrates (\ie, the bitrates which matter), simply using AVC compression with Metabit restoration outperforms deep learning codecs. This is to be expected since Metabit is an objective improvement on AVC which many deep learning methods still struggle to beat in general cases. The advantage of this comes in its ease of use (almost all modern hardware can decode an AVC compressed video) and its speed. Encoding times are in the hundreds of frames-per-second on commodity CPU hardware. Decoding time even including Metabit is also faster.

In \reffig{mb:fps-lc} we compare the throughput of a subset of these methods to Metabit with AVC compression. Metabit is on par with other methods here, and actually outperforms all but NeRV. The major disadvantage of NeRV, however, is the extremely long encoding time. Since NeRV is an implicit representation a new network is learned for each video taking on the order of hours to encode one video. We simply skip encoding time for NeRV in the plot.

The major takeaway from this discussion is that video compression reduction, specifically the Metabit method we developed in this chapter, is efficient and effective at generating accurately restored video frames from low bitrate video. Since it only depends on commodity codecs, our method can be encoded quickly and easily and decoded by anyone without special hardware. Those with special hardware can use our method to achieve more visually pleasing results. This method provides a promising avenue for deploying deep learning in compression in the near term.

\begin{figure*}[t]
    \centering
    \includegraphics{figures/bbb-compare.pdf}
    \caption[Metabit Restoration Example]{\textbf{Metabit Restoration Example.} Crop from $1920 \times 1080$ film ``Big Buck Bunny''. Left: compressed, Middle: restored, Right: Original. This artificial scene is restored accurately despite a lack of artificial training data. Note the grass and tree textures, sharp edges, removal of blocking on the flower, and preservation of the smooth sky region. The video was compressed using AVC CRF 40. }
    \labfig{mb:bbb}
\end{figure*}

==> chapters/video_compression/metabit/future.tex <==
\section{Limitations and Future Work}

The work as presented in this chapter has a few limitation all of which we believe are solvable with relatively minor changes. The network architecture currently depends on a fixed GOP size of seven frames. This would likely not work with real videos which may use a variable length GOP for several reasons. This is readily solvable by projecting a variable size GOP representation to a fixed size one using an adaptive pooling layer following by a projection. It remains to be investigated if this mapping is as effective as using a fixed GOP.

Similarly, since each GOP is treated as a separate block, and restored separately, there are temporal consistency issues across GOP blocks. Note that within a single GOP the frames are quite consistent thanks to the TeCoGAN \sidecite{chu2020learning} formulation which we use. It is only across GOP boundaries that consistency issues arise. This is noticeable in the restored output as a sort of flickering or noise pattern that appears. This is likely solvable by keeping a compact hidden state from the previous GOP to compose with the current GOP processing.

Continuing in this line of thought, there are issues which arise in a streaming scenario which make an architecture like this wholly unsuitable. In streaming scenarios, the video is often encoded using ``low-delay P mode''\index{low-delay p mode}. In this mode, there is a single I-frame at the beginning of the GOP following by only P-frames, in other words, there is only a single GOP in the entire video. For this we actually have a partial solution which is to simply use the previously restored final frame (restored frame 7) in place of the I-frame for the next GOP, skipping the I-frame restoration step entirely. This does lead to a loss of visual quality especially if the network was not trained to perform this kind of restoration.

Another issue in streaming situations is latency and buffering. For real-time applications this currently precludes restoration technology, but in our case in particular the 7 frame GOP needs to be buffered before restoration can occur. This may be a limiting factor in some scenarios. The only way around this is to reduce the number of buffered frames or move to a fully recurrent solution.

Finally, this method suffers from the same ``quality aware'' problem that was prevalent in JPEG artifact correction. For each CRF setting we have to train a different model. Unlike JPEG, however, CRF, and more importantly the derived QP values, are stored in the video file. In this way it should be easy to create a parameterized network which is aware of the QPs that each frame was compressed with.

\begin{figure*}[t]
    \centering
    \includegraphics{figures/mb-compare.pdf}
    \caption[Metabit Comparison]{\textbf{Metabit Comparison.} Crops from ``Big Buck Bunny``'' and ``Traffic'' from the MFQE dataset. We compare our GAN restoration to regression restoration and the STDF method.}
    \labfig{mb:compare}
\end{figure*}

==> chapters/video_compression/metabit/loss.tex <==
\section{Loss Functions}

As we discussed in \nrefch{qgac}, restoration problems which are based purely on regression suffer from blurring and lack low-frequency content. Video compression reduction is no exception to this, and in fact, just like with JPEG compression, video compression specifically removes high frequency content. Unlike other restoration problems, however, all prior work in video compression reduction uses either $l_2$ loss or Charbonnier loss \sidecite{charbonnier1994two}, both of which are simple error penalties. We can introduce more complex loss functions to overcome this. For ``standard`` regression, we will depend on the $l_1$ loss as usual (for the uncompressed frames $X_u$ and the reconstructed frames $X_r$)
\begin{align}
    \Lagr_1(X_u, X_r) = ||X_u - X_r||_1
\end{align}

In \nrefch{qgac}, we were lacking a method for accurate high frequency reconstruction. We can address this here, with partial success, by using a loss based on the Difference of Gaussians (DoG)\index{difference of gaussians} scale space\index{scale space}. The difference of Gaussians constructs a scale space by convolving an image with Gaussian blur kernels of differing standard deviations. These function as bandpass filters which capture image content at different frequency bands. The process is repeated on downsampled versions of the image to capture information at different scales.

We can employ this as a loss function by separating out the different frequency bands at different scales and computing their $l_1$ error as separate loss terms. This effectively weights each frequency band in the same way rather than the decreasing magnitude we see using an overall $l_1$ loss. As such, the network is rewarded for accurately reconstructing high frequencies.

For the uncompressed and reconstructed frames we compute four different scales:
\begin{align}
    S_u = \{X_u, X_{u_2}, X_{u_4}, X_{u_8}\} \\
    S_r = \{X_u, X_{r_2}, X_{r_4}, X_{r_8}\}
\end{align}
where each entry $X_{u_s}$ or $X_{r_s}$ is obtained by downsampling $X_u$ by a factor of $s$. We then compute the difference of Gaussians by convolving with a $5 \times 5$ 2D Gaussian kernel:
\begin{align}
    G(\sigma)_{ij} = \frac{1}{2\pi\sigma^2}e^{-\frac{i^2 + j^2}{2\sigma^2}}
\end{align}
for kernel offsets $i,j$ (note that these range from [-2,2]). Then, for each scale $s$ we compute the four filtered images
\begin{align}
    X_{u_s,\sigma} = G(\sigma) \star X_{u_s} \\
    X_{r_s,\sigma} = G(\sigma) \star X_{r_s}
\end{align}
for $\sigma \in \{1.1,2.2,3.3,4.4\}$. We then compute the differences between the pairs
\begin{align}
    X_{u_s,1} = X_{u_s,2.2} - X_{u_s,1.1} \\
    X_{u_s,2} = X_{u_s,3.3} - X_{u_s,2.2} \\
    X_{u_s,3} = X_{u_s,4.4} - X_{u_s,3.3} \\
    X_{r_s,1} = X_{r_s,2.2} - X_{r_s,1.1} \\
    X_{r_s,2} = X_{r_s,3.3} - X_{r_s,2.2} \\
    X_{r_s,3} = X_{r_s,4.4} - X_{r_s,3.3}
\end{align}
to yield the per-scale frequency bands. Finally, we compute the loss
\begin{align}
    \Lagr_{\text{DoG}}(X_u, X_r) = \sum_{s \in \{1, 2, 4, 8\}}\sum_{b=1}^3||X_{{u_s},b} - X_{{r_s},b}||_1
\end{align}

As in \nrefch{qgac}, however, we find that even this enhanced regression loss is not sufficient to generate realistic reconstructions although it does help. Instead, we again turn to the GAN and Texture losses. The texture loss, repeated here, is discussed at length in \nrefsec{qgac:loss}.
\begin{align}
    \Lagr_t(X_u, X_r) = ||\text{MINC}_{5,3}(X_u) - \text{MINC}_{5,3}(X_r)||_1
\end{align}
where $\text{MINC}_{5,3}$ denotes the output of layer 5 convolution 3 in a MINC \sidecite{bell2015material} trained VGG \sidecite{simonyan2014very} network.

For the GAN loss we will use a Wassertein GAN formulation \sidecite{arjovsky2017wasserstein}. In a Wassertein GAN, the discriminator network is replaced with a critic which rates examples on a [-1, 1] scale with -1 being fake and 1 being real. This critic then makes a soft decision about the realness or fakeness of a sequence rather than a hard decision, which, along with some gradient clipping, makes it more stable and less sensitive to hyperparameter choices.

As in \nrefch{qgac} our critic architecture is based on DCGAN \sidecite{radford2015unsupervised} with spectral normalized convolutions \sidecite{miyato2018spectral} except that we modify the critic procedure to introduce temporal consistency following the procedure from TeCoGAN \sidecite{chu2020learning}. The modification is relatively simple: we use the compressed and restored/uncompressed sequence as input with the frames stacked in the channel dimension. The means the critic is now considering the entire sequence instead of individual frames and therefore is incentivised to produce similar reconstructions over the sequence. The architecture is shown in \reffig{mb:critic}. This yields the GAN loss
\begin{align}
    \Lagr_w(X_u, X_r) = -d(X_u,X_r)
\end{align}
for critic $d()$ \sidenote{Note that the critic itself has a different loss function which we do not show here, see \cite{arjovsky2017wasserstein} for details.}.
\begin{marginfigure}
    \centering
    \includegraphics{figures/critic.pdf}
    \caption[Metabit Critic Architecture]{\textbf{Metabit Critic Architecture.} For the entire seven frame sequence, the compressed and restored frames are concatenated following \parencite{chu2020learning}. The resulting 48 channel input is reduced to a single scalar using a series of spectral-normed convolutions, batch norm, and ReLU layers.}
    \labfig{mb:critic}
\end{marginfigure}

These are combined into two composite loss functions: one for regression only results
\begin{align}
    \Lagr_R(X_u, X_r) = \bm{\alpha}[\Lagr_1(X_u, X_r)\; \Lagr_\text{DoG}(X_u, X_r)]^T
    \labeq{mb:regloss}
\end{align}
for balancing hyperparameters $\bm{\alpha} \in \mathbb{R}^2$ and a loss for qualitative results
\begin{align}
    \Lagr_G(X_u, X_r) = \bm{\beta}[\Lagr_1(X_u, X_r)\; \Lagr_\text{DoG}(X_u, X_r)\;  \Lagr_W(X_u, X_r)\; \Lagr_t(X_u, X_r)]^T
    \labeq{mb:ganloss}
\end{align}
for balancing hyperparameters $\bm{\beta} \in \mathbb{R}^4$.

==> chapters/video_compression/metabit/tables/gan.tex <==
\begin{tabular}{@{}rll@{}}
    \toprule
    \multirow{2}{*}{Method} & \multicolumn{2}{c}{H.264 CRF}                                     \\
    \cmidrule{2-3}          & 40                            & 50                                \\
    \midrule
    AVC                   & 67.07 / 0.259                 & 152.19 / 0.498                    \\
    Regression              & 80.67 / 0.265                 & 154.42 / 0.482                    \\
    \textbf{GAN}            & \textbf{37.78 / 0.191}        & \textbf{\phantom{0}95.26 / 0.368} \\
    \bottomrule
\end{tabular}

==> chapters/video_compression/metabit/tables/h264.tex <==
\begin{tabular}{@{}rllll@{}}
    \toprule
    \multicolumn{1}{c}{\multirow{2}{*}{Method}}        & \multicolumn{4}{c}{AVC CRF}                                                                               \\
    \cmidrule{2-5}                                     & 25                          & 35                     & 40                      & 50                       \\
    \midrule
    STDF-R1 \parencite{Deng_Wang_Pu_Zhuo_2020}         & 0.741 / 0.034               & 0.862 / 0.032          & 0.814 / 0.030           & 0.632 / \phantom{-}0.013 \\
    STDF-R3 \parencite{Deng_Wang_Pu_Zhuo_2020}         & 0.784 / 0.035               & 0.846 / 0.032          & 0.882 / 0.029           & 0.817 / \phantom{-}0.011 \\
    \textbf{MetaBit} \parencite{ehrlich2022leveraging} & \textbf{1.085 / 0.024}      & \textbf{1.137 / 0.014} & \textbf{1.113 / 0.005 } & \textbf{0.887 / -0.016 } \\
    \bottomrule
\end{tabular}

==> chapters/video_compression/metabit/tables/h265.tex <==
\begin{tabular}{@{}rllll@{}}
    \toprule
    \multicolumn{1}{c}{\multirow{2}{*}{Method}}          & \multicolumn{4}{c}{HEVC CQP}                                                                     \\
    \cmidrule{2-5}                                       & 27                           & 32                    & 37                    & 42                \\
    \midrule
    MFQE 2.0 \parencite{Xing_Guan_Xu_Yang_Liu_Wang_2021} & 0.49 / -                     & 0.52 / -              & 0.56 / -              & 0.59 / -          \\
    PSTQE \parencite{ding2021patch}                      & 0.63 / -                     & 0.67 / -              & 0.69 / -              & 0.69 / -          \\
    STDF-R3 \parencite{Deng_Wang_Pu_Zhuo_2020}           & 0.72 / \textbf{0.025}        & 0.86 / 0.027          & 0.83 / 0.033          & - / -             \\
    RFDA \parencite{zhao2021recursive}                   & 0.82 / -                     & 0.87 / -              & \textbf{0.91} / -     & \textbf{0.82} / - \\
    \textbf{MetaBit} \parencite{ehrlich2022leveraging}   & \textbf{1.17 / 0.025}        & \textbf{0.99 / 0.023} & \textbf{0.91 / 0.029} & \textbf{0.82} / - \\
    \bottomrule
\end{tabular}

==> front/acknowledgements.tex <==
\noindent Special thanks to
\begin{itemize}
    \item \href{https://q4.github.io/}{Christian Steinruecken} for providing the math coloring function from his \href{https://q4.github.io/thesis.html}{dissertation.}
    \item My editors: \href{https://www.cs.umd.edu/~shishira/}{Shishira Maiya}, \href{https://lilhuang.github.io/about/}{Lillian Huang}, \href{https://www.linkedin.com/in/vatsalag99/}{Vatsal Agarwal}, and \href{https://www.linkedin.com/in/namitha-padmanabhan-a8b0121b3/}{Namitha Padmanabhan}.
    \item My social media consultant \href{https://somepago.github.io/}{Gowthami Somepalli} and her assistant \href{https://kampta.github.io/}{Kamal Gupta}.
\end{itemize}

\noindent The research presented in this dissertation was partially supported by Facebook AI, Defense Advanced Research Projects Agency (DARPA) MediFor (FA87501620191), DARPA SemaFor (HR001119S0085) and DARPA SAIL-ON (W911NF2020009) programs. There is no collaboration between Facebook and DARPA.

==> front/copyright.tex <==
\makeatletter
\uppertitleback{\@titlehead} %

\lowertitleback{
    \textbf{Disclaimer}\\
    This document was created for partial fulfillment of the requirements of the degree of Doctor of Philosophy in Computer Science and therefore does not purport to impart any knowledge of any particular subject. Any knowledge obtained as as result of reading this document is entirely coincidental and should be used at the readers own risk.

    \medskip

    \textbf{Copyright}\\
    Copyright \copyright \hbox{ } 2022 Max Ehrlich

    \medskip

    \textbf{License} \\
    \input{front/license.tex}

    \medskip

    \textbf{Acknowledgement} \\
    This document was typeset with the help of \href{https://sourceforge.net/projects/koma-script/}{\KOMAScript} and \href{https://www.latex-project.org/}{\LaTeX} using the \href{https://github.com/fmarotta/kaobook/}{kaobook} class. \\

    \input{front/acknowledgements}

    \medskip

    \textbf{Publisher} \\
    Self-published electronically in April 2022. \url{https://maxehr.umiacs.io/dissertation}.
}
\makeatother

==> front/license.tex <==
The First Principles of Deep Learning and Compression is licensed under the Creative Commons \href{https://creativecommons.org/licenses/by-nc-nd/4.0/?ref=chooser-v1}{Attribution-NonCommercial-NoDerivatives 4.0 International} license. \\
CC BY-NC-ND 4.0 \ccbyncnd
